ClipCap: CLIP Prefix for Image Captioning

Image captioning is a fundamental task in vision-language understanding, where the model predicts a textual informative caption to a given input image. In this paper, we present a simple approach to address this task. We use CLIP encoding as a prefix to the caption, by employing a simple mapping network, and then fine-tunes a language model to generate the image captions. The recently proposed CLIP model contains rich semantic features which were trained with textual context, making it best for vision-language perception. Our key idea is that together with a pre-trained language model (GPT2), we obtain a wide understanding of both visual and textual data. Hence, our approach only requires rather quick training to produce a competent captioning model. Without additional annotations or pre-training, it efficiently generates meaningful captions for large-scale and diverse datasets. Surprisingly, our method works well even when only the mapping network is trained, while both CLIP and the language model remain frozen, allowing a lighter architecture with less trainable parameters. Through quantitative evaluation, we demonstrate our model achieves comparable results to state-of-the-art methods on the challenging Conceptual Captions and nocaps datasets, while it is simpler, faster, and lighter. Our code is available in https://github.com/rmokady/CLIP_prefix_caption.

==> images/teaser_horizontal.tex <==
\vspace*{-0.5cm}
\bgroup

\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{3pt}

  \centering
  \footnotesize
\begin{tabular}{p{\imagew} p{\imagew} p{\imagew}  p{\imagew}}


%\includegraphics[width=\imagew,height=\imageh]{images/IMG_2039.jpg}
\includegraphics[width=\imagew,height=\imageh]{images/yoga.jpeg} &
\includegraphics[width=\imagew,height=\imageh]{images/automn.png} &
%\includegraphics[width=\imagew,height=\imageh]{images/Yayoi_Kusama_Pumpkin_foto.jpg} &
\includegraphics[width=\imagew,height=\imageh]{images/Merkel_an_Obama.jpeg} &
\includegraphics[width=\imagew,height=\imageh]{images/bow-ties.jpg} \\
%A person standing in front of a rock formation in the desert. & The pumpkin is a symbol of the season. &
%A politician receives a gift from politician. & Silhouette of a woman practicing yoga on the beach at sunset. 
Silhouette of a woman practicing yoga on the beach at sunset. & Aerial view of a road in autumn. & A politician receives a gift from politician. & A collage of different colored ties on a white background. \\
%\vspace*{0.2cm}\\

%\includegraphics[width=\imagew,height=\imageh]{images/Gorilla.png} &
%\includegraphics[width=\imagew,height=\imageh]{images/automn.png} &
%\includegraphics[width=\imagew,height=\imageh]{images/bow-ties.jpg} &
%\includegraphics[width=\imagew,height=\imageh]{images/The_Parthenon_in_Athens.jpg} \\
%  A cartoon illustration of a gorilla looking angry. & Aerial view of a road in autumn. &
%  A set of striped ties for men and women. & Temple of deity in the ruins.  
\end{tabular}
%\end{center}

\captionof{figure}{
%Given an image as input, our model produce captions depicting those photos. In this figure, our model was trained over Conceptual Captions dataset, therefore the captions do not specify entities (e.g. Obama) rather focus on the concept similarly to the dataset samples. 
%\dc{I suggest displaying a single row with t examples. And change the caption to be less defensive:} 
Our ClipCap model produces captions depcting the respective images. Here, the results are of a model that was trained over the Conceptual Captions dataset.}
\vspace*{0.4cm} 
\label{fig:teaser} 
\egroup

==> images/union_caption_examples.tex <==
\captionsetup[subfigure]{font=normalsize, justification=justified,singlelinecheck=false}
\begin{figure*}
\footnotesize
\begin{subfigure}{\columnwidth}
\centering


\subcaption{\textbf{COCO}}
\vspace{-.2cm}
\begin{tabular}{p{0.2\columnwidth} p{0.33\columnwidth}p{0.33\columnwidth}p{0.33\columnwidth}p{0.33\columnwidth}p{0.32\columnwidth}}
&
\includegraphics[trim={2cm 0 0 0},clip,width=0.34\columnwidth,height=0.22\columnwidth]{images/COCO_val2014_000000391895.jpg} &
\includegraphics[width=0.34\columnwidth,height=0.22\columnwidth]{images/COCO_val2014_000000060623.jpg} &
\includegraphics[trim={0, .1cm 0 .2cm},clip,width=0.34\columnwidth,height=0.22\columnwidth]{images/COCO_val2014_000000483108_crop.jpg} &
\includegraphics[trim={0 10cm 0 2cm},clip,width=0.34\columnwidth,height=0.22\columnwidth]{images/COCO_val2014_000000386164.jpg} &
\includegraphics[trim={0 1cm 0 1cm},clip,width=0.34\columnwidth,height=0.22\columnwidth]{images/COCO_val2014_000000384213.jpg} \\
% \hline
\begin{tabular}{l}Ground Truth \end{tabular}& A man with a red helmet on a small moped on a dirt road & A young girl inhales with the intent of blowing out a candle.  
& A man on a bicycle riding next to a train. & a wooden cutting board topped with sliced up food.  & A kitchen is shown with a variety of items on the counters.\\
\hline
\begin{tabular}{l}Oscar \end{tabular}& a man riding a motorcycle down a dirt road. & a woman sitting at a table with a plate of food.  & a woman riding a bike down a street next to a train. & a woman sitting at a table with a plate of food.  & a kitchen with a sink, dishwasher and a window.\\
\hline
\begin{tabular}{l}
Ours-- \\ with tuning 
\end{tabular}& a man riding a motorcycle on a dirt road. & a woman is eating a piece of cake with a candle. & a man is standing next to a train. & a row of wooden cutting boards with wooden spoons. & a kitchen with a sink, stove, and window.\\
\hline
\begin{tabular}{l}
Ours-- \\ w/o tuning
\end{tabular}  & a man is riding a motorbike on a dirt road. & a young girl sitting at a table with a cup of cake. &  a man is standing next to a train.  & a wooden table with a bunch of wood tools on it.   & a kitchen with a sink and a window. \\

\end{tabular}


\label{fig:img} 

\end{subfigure}

\vspace{.2cm}

\begin{subfigure}{\columnwidth}
\subcaption{\textbf{Conceptual Captions}}

\centering
\begin{tabular}{p{0.2\columnwidth} p{0.33\columnwidth}p{0.33\columnwidth}p{0.33\columnwidth}p{0.33\columnwidth}p{0.33\columnwidth}}
&
\includegraphics[trim={0 3cm 0 2cm},clip,width=0.34\columnwidth,height=0.24\columnwidth]{images/00.jpg} &
\includegraphics[trim={0 2cm 0 0},clip,width=0.34\columnwidth,height=0.24\columnwidth]{images/01_crop.jpg} &
\includegraphics[trim={0 .1cm 0 .2cm},clip,width=0.34\columnwidth,height=0.24\columnwidth]{images/03_crop.jpg} &
\includegraphics[width=0.34\columnwidth,height=0.24\columnwidth]{images/02.jpg} &
\includegraphics[width=0.34\columnwidth,height=0.24\columnwidth]{images/04.jpg} \\

% \hline
\begin{tabular}{l}Ground Truth \end{tabular}& A life in photography -- in pictures. & Photograph of the sign being repaired by brave person. 
& Globes : the green 3d person carrying in hands globe. &  The player staring intently at a computer screen.  & The - bedroom stone cottage can sleep people.\\
\hline
\begin{tabular}{l}VLP \end{tabular}&  Actors in a scene from the movie. & The sign at the entrance.  & Templates: green cartoon character holding the earth globe. & Person works on a video.  &  The master bedroom has a king - sized bed with a queen size bed.  \\
\hline
\begin{tabular}{l}
Ours-- \\ with tuning 
\end{tabular}& Actor sits in a hotel room. & The sign at the entrance. & 3d render of a man holding a globe. & Person, a student, watches a video on his laptop.  & The property is on the market for £ 1.\\
\hline
\begin{tabular}{l}
Ours-- \\ w/o tuning 
\end{tabular}& person sitting on a chair in a room. & a sign is seen at the entrance to the store. & stock image of a man holding the earth. & portrait of a young boy playing video game. & one of the bedrooms in the house has been converted into a living room. 
\end{tabular}

\label{fig:img_conceptual} 
\end{subfigure}

\vspace{-.3cm}
\caption{Uncurated results of the first five images in COCO test set (Karpathy et al.~\cite{karpathy2015deep} split) and in the Conceptual Captions validation set \cite{sharma2018conceptual}.}

 \label{fig:caption_examples}
\end{figure*}






